ThundeRiNG: Generating Multiple Independent Random Number Sequences on FPGAs

In this paper, we propose ThundeRiNG, a resource-efficient and high-throughput system for generating multiple independent sequences of random numbers (MISRN) on FPGAs. Generating MISRN can be a time-consuming step in many applications such as numeric computation and approximate computing. Despite that decades of studies on generating a single sequence of random numbers on FPGAs have achieved very high throughput and high quality of randomness, existing MISRN approaches either suffer from heavy resource consumption or fail to achieve statistical independence among sequences. In contrast, ThundeRiNG resolves the dependence by using a resource-efficient decorrelator among multiple sequences, guaranteeing a high statistical quality of randomness. Moreover, ThundeRiNG develops a novel state sharing among a massive number of pseudo-random number generator instances on FPGAs. The experimental results show that ThundeRiNG successfully passes the widely used statistical test, TestU01, only consumes a constant number of DSPs (less than 1\% of the FPGA resource capacity) for generating any number of sequences, and achieves a throughput of 655 billion random numbers per second. Compared to the state-of-the-art GPU library, ThundeRiNG demonstrates a $10.62\times$ speedup on MISRN and delivers up to $9.15\times$ performance and $26.63\times$ power efficiency improvement on two applications ($\pi$ estimation and Monte Carlo option pricing). This work is open-sourced on Github at https://github.com/Xtra-Computing/ThundeRiNG

==> 3_thm_3.tex <==
%!TEX root = main.tex

\begin{theorem} \label{thm:3}

Considering a LCG transition, which is defined as $x_{n+1} = a \cdot x_{n} + c \pmod{ m }$, and an addition transition, which is defined as $ w^{n + 1} = x^{n + 1} + h \pmod {m}$. The transition between $w^{n + 1}$ and $w^{n}$ is also a LCG transition.

%The combined transition is equal to another LCG transition.


\end{theorem}
\begin{proof}[Proof]

We give a deduction as follows: 
    \begin{align*}
    w_{n } &= (x_{n} + h)\Mod{m} = x_{n} + h + l \cdot m \\
    w_{n + 1} &= (x_{n+1} + h)\Mod{m} \\
     &= a \cdot x_{n} + c  + h + l' \cdot m \\
     &= a (x_n + h + l \cdot m) - a \cdot h + c + (l' - a \cdot l) m \\
     &= a \cdot w_n + (l'' \cdot m + c - a \cdot h) + (l' - a \cdot l - l'') m \\
     &= [a \cdot w_n + (l'' \cdot m + c - a \cdot h)] \Mod{m}  \qedhere
    % \therefore   W &= X_{a,m}^{(l'' \cdot m + c - a \cdot h)} \Rightarrow  W \in \mathbb{X}_{a,m}
    \end{align*} 
    Where we can see that the transition between $w_{n + 1}$ and $w_{n}$ is with the same form of LCG. \qedhere
    %Hence, $w_{n + 1} = (a \cdot  w_n + c')\Mod{m}$, where the $c'$ is equal to 
    %$l'' \cdot m + c - a \cdot h$ is a form of LCG transition.
    

\end{proof}

==> commented/1-introduction-v1.tex <==
%!TEX root = main.tex
\section{introduction}\label{sec:int}
Pseudo-random number generator (PRNG), which generates a sequence of numbers whose properties approximate the properties of sequences of random numbers, is of great importance for computer simulation, numerical analysis, and modeling.
Examples include Monte Carlo simulation and approximated graph mining~\cite{quoc2017approximate,222637,pavan2013counting}.
With the scaling of problem size and the need of parallelization of these applications, the development of high throughput and high-quality PRNGs on modern hardware has attracted increased attention.

%In order to elaborate the design gap better, we introduce two successive stages of PRNGs in the below equation:
Normally, RPNG consists of two successive stages: state transition and output, to generate random numbers, as shown in the following equations:
%~\Cref{eq:def1,eq:def2};
\begin{align}
s_n &= f(s_{n-1}),~ n=1,2,3, \ldots \label{eq:def1}\\
u_n &= g(s_n) \label{eq:def2}
\end{align}
where the $ f \colon \boldsymbol{S} \to \boldsymbol{S} $ is the state transition function which maps an state $s_n$ to next state $s_{n+1}$ in the state space $\boldsymbol{S}$, and $ g \colon \boldsymbol{S} \to \boldsymbol{U} $ is the output function that extracts a number in the output space $\boldsymbol{U}$ according to a given state.
In order to generate sequences with high-quality randomness, the state transition function is carefully crafted and complicated, and the output function usually includes bit-wise operations such as truncation or permutation.
%then enhances the quality by solving flaws existing in the state sequence.
%It is noteworthy that the output function usually evolve bit-wise permutation for.

Given the computation pattern of PRNGs, Field programmable gate arrays (FPGAs) demonstrate unprecedented architectural advantages compared to CPUs and GPUs when extracting parallelism of PRNGs.
Usually, CPUs and GPUs adopt Single Instruction Multiple Data (SIMD) instruction and multi-threading~\cite{saito2008simd} for parallelization.
However, they are not efficient for PRNGs.
Firstly, the bit permutation operations such as random rotation~\cite{o2014pcg} lack dedicated instructions on modern processor architectures and hence needs to combine multiple bit-wise instructions, decreasing the performance.
Secondly, PRNGs always involve large integer arithmetic (e.g., data with 1024-bit~\cite{blackman2018scrambled}) or non-aligned arithmetic (96-bits), which can only be assembled by multiple lower-bit math instructions.
% I feel these two points can be combined together....  discuss it later.
Lastly, the PRNG and application-specific processing logic are two independent tasks in general, for the PRNG which has large state space, it introduces a large overhead in the context switching causing severe cache thrashing~\cite{passerat2011pseudo}.
On contrast, being able to customize hardware logic in bit level, the algorithm-specific permutation can be pipelined with high throughput, the large-bit or arbitrary integer arithmetic can be efficiently implemented on FPGAs.
The processing logic and RRNG can be pipelined.
%Besides, FPGAs which have ultra high on-chip memory bandwidth and the ability of fine-grain parallelism enable the customized long pipeline for both PRNG and application processing logic. Hence, FPGA is becoming an attractive platform for applications requiring high throughput PRNGs.

%Exiting methods either have quality but no high throughput or high throughput no quality.
Despite architectural advantages, existing FPGA-based PRNGs still suffer several problems.
It is noteworthy the throughput of a single generator is limited due to the inherent sequential natural of the PRNGs algorithm: the state is generated from the previous one (as shown in Equation~\ref{eq:def1}).
Therefore, the common approach for paralleling the RPNGs is to increase the number of independent PRNG instances to generate multiple uncorrelated sequences at the same time.
%There are several challenges for the concurrent generation of multiple random number sequences on FPGAs.
%PRNGs which can generate high-quality independent sequences are hard to find~\cite{hellekalek1998good}. More importantly, the limited resources on hardware platforms constrains the maximum number of PRNG instances.

In~\Cref{tab:cost_prng}, we survey state-of-the-art FPGA-based PRNG algorithms and implementations (the details will be explained in~\Cref{sec:related_work}).
The statistics conclude that existing FPGA-based PRNGs could not satisfy the ``high quality'' and ``high throughput'' criteria at the same time.
Their weaknesses can be classified into two categories:

\input{table_1}


\noindent
\textbf{High throughput but low quality}.
There exists a class of high throughput RPNGs on FPGAs, binary linear generators~\cite{thomas2012lut,comer2012random,thomas2008fpga,knuth2014art}, whose state transition function is specifically optimized for the logic cells in FPGA can efficiently utilize the hardware resources. However, all of them are based on linear recurrence which are proven to have problem on linear complexity, hence prohibiting them from applications that need high-quality random number sequences.

\noindent
\textbf{High quality but low throughput}.
Existing PRNGs on FPGAs with high-quality randomness are resource unfriendly.
Some of them adopt a complicated state transition function, for example, increasing the space of state~\cite{matsumoto1998mersenne} or introducing non-linear arithmetic~\cite{dabal2014study,dabal2012fpga}.
Meanwhile, many others instead embrace simple state transition function~\cite{blackman2018scrambled,salmon2011parallel} and adopt a intricate scramble of state in output stage. However, the high-quality scramble requires multiply arithmetic.
Therefore, in the context of concurrent random number generation which requires to instance massive number of PRNGs, all of the high-quality PRNGs leads to a proportional consumption of precision resources. More detailed, they occupy either a large portion of BRAMs for storing the state or huge number of DSP resources for non-linear transformation.
As a result, the number of independent PRNG instances on FPGA is limited, violating the high throughput criteria.


%In summary, FPGA based high throughput PRNGs with high quality is still hard to find.
%In order to make good use of FPGA in applications requiring PRNGs,

In this paper, we propose \textit{ThunderRiNG}, which brings both ``high quality'' and ``high throughput'' for FPGA-based PRNGs.
ThunderRiNG is based on linear congruential generator (LCG) because that it has been well-studied in theory~\cite{durst1989using,o2014pcg,l1999tables}.
%ThunderRiNG is the FPGA-based implementation of our multiplication-insensitive multiple sequence PRNG.
% in the next, we introduce what we have done.
In order solve the resource inefficiency problem for increasing the number of PRNGs instanced on FPGAs, we propose a state sharing mechanism, which uses a single state transition function for the generating multiple independent sequences. Therefore, the consumption of DSPs is oblivious to the number of independent instances, the state is efficiently reused among a large number of instances by the flexible on-chip routing which is enabled by FPGA architecture.
%Instead of only focusing on the specific optimization with the structure of logic unit on modern FPGAs,
More importantly, to provide high quality, we propose a lightweight and resource efficient decorrelation mechanism to solve the correlation introduced by the reuse of state. The theoretical analysis and experimental results demonstrate that our approach brings significant improvement on the statistical quality and achieves high throughput with efficient resource utilization.

In summary, this paper makes the following contributions:
\begin{itemize}[leftmargin=*]

%\item We propose a new parameterization method for LCGs to generate multiple statistical independent random sequences by coupling with a decorrelation process. (?)

\item We present a resource-efficient generation mechanism called state sharing, which is based on the existing multistream approach and enables the reuse of state over a decorrelation method.

\item We adopt an efficient implementation of the above method on FPGA platform, the throughput of generation is up to 20.9Tb/s.

\item We demonstrate the effectiveness of our design on two real world applications. Results show that our FPGA implementation delivers up to 6.87x speedup on throughput and 15.25x power efficiency when compared to state-of-the-art GPU based PRNGs.

\end{itemize}


==> commented/5-evaluation-legacy.tex <==
%!TEX root = main.tex

\section{Evaluation}\label{sec:eva}

\todo[inline]{Add in the resource consumption of the state in the single sequence generation.}

In this section, we evaluate ThundeRiNG over existing RNGs on statistical quality and throughput, followed by two real applications to demonstrate the effectiveness of ThundeRiNG.


\subsection{Experimental Setup}
\subsubsection{Hardware Platform}
The evaluation of statistical quality is conducted on a server with Intel Xeon 6288 CPU and 768 GB memory.
The hardware implementations of ThundeRiNG and two applications are on a Xilinx Alveo U250 accelerator card.
The FPGA device has 2301 BRAMs and 12272 DSP slices, the development tool is Vitis HLS 2020.1.
%The target GPU device is NVIDIA Tesla P100 on a server with Intel Xeon E5-2640 CPU inside.


\subsubsection{Evaluating the Statistical Quality} \label{subsec:randomness_test}
%it is widely These tests rely on the null hypothesis testing of the statistic properties of input sequences with the assumption of i.i.d.
%\subsubsection {Empirical testing}

\noindent
\textbf{TestU01 suite.}
Although several empirical test suites for PRNGs have been proposed, the most complete and stringent test is the TestU01 suite\cite{l2007testu01}, whose batteries of randomness tests include not only earlier suites~\cite{bassham2010sp,marsaglia1995diehard} but also tests from other sources\cite{takashima1996last,erdmann1992empirical} that are not incorporated into a test suite.
%
The commonly used systemic batteries in TestU01 include SmallCrush (10 tests), Crush (96 tests), and BigCrush (160 tests).
PRNGs that pass all tests in those batteries can be referred as \textbf{\textit{crush-resistant}} while the PRNGs fail to do that is called \textbf{\textit{crushable}}~\cite{salmon2011parallel}.
A crushable PRNG definitively indicates that it has recognizable patterns, whose quality should be carefully considered in applications.
%It is noteworthy that a crush-resistant PRNG can be to be flawless.
%Note that, A crush-resistant PRNG can never prove it is flawless, but if there are failed tests, it definitively indicates that there are known patterns existing in this generation algorithm which should be carefully considered in applications.


We evaluate intra-stream and inter-stream correlations of ThundeRiNG. The testing on the intra-stream is conducted by TestU01, and we judge the quality using the criteria from~\cite{salmon2011parallel}.
%following the commonly used criteria and method which has been introduced in~\Cref{subsec:randomness_test}, and
We further comprehensively evaluate inter-stream correlations in following aspects: systematic evaluation, pairwise correlations and Hamming weight dependency.

The systematic evaluation is conducted in following steps. Firstly, we select number of sequences at random, and then combining these sequences into one sequence:
the $k$ sequences, which can be represented by: $\{x^{i}_{0}, x^{i}_{1}, ..., x^{i}_{n},...\}$, where the $i$ is the unique index of distinct sequences, are interleaved into a new sequence $\{x^{0}_{0},x^{1}_{0},...,x^{k}_{0},x^{0}_{1},x^{1}_{1},...\}$. Finally, BigCrush battery is applied to this sequence. This interleaving scheme is same with the pattern that the random numbers are consumed. Therefore, if there is failure from BigCrush, it indicates a kind of inter-stream correlation is detected. As up to 160 testing aims different types of regular patterns are conducted in BigCrush
The final result systematically represents that to what extent the streams are correlated with each other.

To evaluate the effectiveness of our decorrelation approach, we further analyze the pairwise correlation. Pearson’s correlation coefficient, Spearman’s rank correlation coefficient, and Kendall’s rank correlation coefficient is considered.
The Pearson correlation is also known as the cross-correlation, and it is a measure of the strength of the linear relationship between two sequences, and if the Pearson correlation is close to zero, it indicates the two sequences are not linearly correlated with each other. Spearman’s rank correlation represents the strength and direction of the monotonic relationship between two variables, and it is commonly used when the assumptions of the Pearson correlation are markedly violated. Kendall rank correlation is a statistic used to measure the ordinal association between two measured quantities, it describes the similarity of the orderings of the data when sorted by each of the quantities. As it is hard to traverse and analyze the pairwise correlations of all candidate sequences, we randomly select two distinct sequences to calculate the three coefficient and report the maximal number over numbers of iterations.

As the state is reused in the generation of all the sequences, it brings the Hamming weight dependencies among the sequences which are undetectable by the pairwise correlation coefficients. Therefore, we adopt the state-of-the-art Hamming weight dependencies testing(HWD)~\cite{blackman2018scrambled} to further evaluate the generated sequences. the HWD testing is conducted on the interleaved sequence which is the same as the one using in systematic evaluation.


%compare with GPU-based RNGs on Nvidia Tesla P100 with CUDA 10.2..

\subsection{Statistical Quality Evaluation}
\subsubsection{Systematic Evaluation}
We first follow the standard of ``crush-resistant'' (in~\Cref{subsec:randomness_test}) to evaluate the statistical properties of single sequence and multiple sequences and make comparison with the state-of-the-art PRNG algorithm.
%The multiple sequences testing~\cite{li2011software} is conducted by interleaving distinct streams into one single stream and then testing the new stream in BigCrush battery from TestU01.
Testing results in~\Cref{tab:overall_statistic_results} show that ThundeRiNG passes all tests.
The sequences generated by ThundeRiNG have the same quality of statistical randomness and independence with the sequences of state-of-the-art algorithms.
%and the dependence among multiple sequences is not detected by the

\begin{table}[h!]
\caption{Statistical testing on ThundeRiNG and state-of-the-art PRNG algorithms}
\label{tab:overall_statistic_results}
\resizebox{0.486\textwidth}{!}{%
\begin{tabularx}{0.7\textwidth}{lcccc}
\toprule

\multirow{1}{*}{\textbf{Algorithms}}
& \multirow{1}{*}{\textbf{ThundeRiNG}}
& \multirow{1}{*}{\textbf{Philox-4×32~\cite{salmon2011parallel}}}
& \multirow{1}{*}{\textbf{SplitMix~\cite{steele2014fast}}}
& \multirow{1}{*}{\textbf{MRG32k3a~\cite{l1999good}}}
\\
\midrule

\multirow{1}{*}{{Single sequence}} & \textbf{Pass} & Pass & Pass & Pass        \\
\multirow{1}{*}{{Multi-sequences}}& \textbf{Pass} & Pass & Pass & 1 failure \\

\bottomrule

\end{tabularx}%
}
\end{table}



\subsubsection{Detailed evaluation} \label{subsubsec:details}

We further evaluate the individual efficacy of decorrelation and permutation with the cross-correlation analysis and Hamming weight dependency testing~\cite{blackman2018scrambled}, as shown in~\Cref{tab:correlation_results}.
Cross-correlation is a common metric for the similarity of two sequences, and a smaller value indicates a higher quality on dependency.
We randomly select two distinct sequences to calculate cross-correlation and report the maximal number over 1000 times iterations.
%The reason of conducting Hamming weight dependence testing is that the similarity in
%If the streams are independent with each other, the cross-correlation should be close to zero.
%The cross-correlation is measured by iteratively calculating it[??] between two randomly selected distinct sequences and reported with the maximal number over 1000 times testings.
%Hamming weight is another well-known and commonly used metric for......
As the state which has the same Hamming weight is reused among many instances, there is potential statistical bias in the Hamming weight of different sequences.
Therefore, we conduct the latest Hamming weight dependency (HWD) testing from~\cite{blackman2018scrambled} to discover more bias patterns of HWD than the BigCrush.
The result of HWD testing indicates the number of generated random numbers before an unexpected pattern is detected, hence the higher value the better.
In addition, the BigCrush for multiple sequences is also presented for each method.

\begin{table}[h!]
\caption{Correlation and dependence evaluations on our proposed method}
\label{tab:correlation_results}
\resizebox{0.476\textwidth}{!}{%
\begin{tabularx}{0.65\textwidth}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Combined algorithms}}
& \multirow{2}{*}{\textbf{Cross-correlation}}
& \multirow{2}{*}{\textbf{HWD test~\cite{blackman2018scrambled}}}
& \multirow{1}{*}{\textbf{Multi-sequences}}
\\
&
&
& \multirow{1}{*}{\textbf{BigCrush}}
\\
\midrule

LCG                         & 0.97            & $ < 1.25e+08 $     &  146                \\
LCG with Decorrelation      & 0.0046          & $ > 1e+14$         &  4                  \\
LCG with Permutation        & 0.0041          & $ < 1.25e+08 $     &  105                \\
\textbf{ThundeRiNG}         & \textbf{0.0032} & $\mathbf{> 1e+14}$ & \textbf{0}          \\
\bottomrule

\end{tabularx}%
}

\end{table}

The results show that the original LCG (parameterization via increment but without decorrelation) has high correlation and fails on almost all tests in BigCrush.
With only applying the decorrelation to LCG, the cross-correlation decreases from 0.97 to 0.0046, and there is no sign of Hamming weight bias even after 100 trillions of random numbers, which is much bigger than LCG (125 million).  It demonstrates that our proposed decorrelation method (in~\Cref{subsec:decorrelation}) significantly improves the independence of multiple sequences. However there are still 4 failures in BigCrush testing, and these failures are related with the statistical flaws of low-order bits.
With only applying the permutation, the cross-correlation has reduced because the nonlinearity introduced by permutation also reduces the similarity.
However, there is no improvement on Hamming weight dependence since the bijective remapping in permutation does not change the Hamming weight.
Combined permutation and decorrelation together, our ThundeRiNG passes all tests and shows smaller cross-correlation.

\subsection{The Selection of LCG and Decorrelator} \label{subsubsec:selection_of_decorr}



\begin{table}[h!]
\caption{The comparison of LCG with different bit width}
\label{tab:selection_of_lcg}
\resizebox{0.476\textwidth}{!}{%
\begin{tabularx}{0.63\textwidth}{lrcc}
\toprule

\multirow{1}{*}{\textbf{Bits }}
& \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Multiplicative constant [$a$ in~\Cref{eq:lcg}] }}}
& \multirow{1}{*}{\textbf{Period}}
& \multirow{1}{*}{\textbf{DSP cost}}
\\
\midrule

64                    & 9199940308585234877                      &  $2^{64} - 1$  &  10      \\
72 ($36\times2$)      & 1277974755392284889725                   &  $2^{72} - 1$  &  13      \\
96                    & 61124247442928732736190063229            &  $2^{96} - 1$  &  21      \\
108 ($36\times3$)     & 303587630294941123502336685825389        &  $2^{108} - 1$ &  26      \\
128                   & 199967246047888932297834045878657099405  &  $2^{128} - 1$ &  34      \\
\bottomrule

\end{tabularx}%
}

\end{table}


\begin{table}[h!]
\caption{The comparison of different decorrelator}
\label{tab:selection_of_decorr}
\resizebox{0.476\textwidth}{!}{%
\begin{tabularx}{0.6\textwidth}{lcccc}
\toprule

\multicolumn{3}{c}{\multirow{1}{*}{\textbf{Decorrelator}}}
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Maximum degree of parallelism}}}
\\ \cline{1-3}

\multirow{2}{*}{\textbf{Algorithms}}
& \multirow{1}{*}{\textbf{Systematic}}
& \multirow{1}{*}{\textbf{Resources}}
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{(Crush-resistant)}}}
\\ \cline{4-5}


& \multirow{1}{*}{\textbf{Failures}}
& \multirow{1}{*}{\textbf{(LUT + FF)}}
& \multirow{1}{*}{\textbf{Theoretical}}
& \multirow{1}{*}{\textbf{Evaluated}}
\\
\midrule

xorshift32      & 75  &  275   &  1             &     $2^{12}$       \\
xorshift64      & 32  &  563   &  1             &     $2^{16}$       \\
xorshift128     & 7   &  1125  &  $2^{64}$      &    up to $2^{32}$  \\
xorwow          & 20  &  2076  &  $2^{128}-1$   &    up to $2^{32}$  \\
\bottomrule

\end{tabularx}%
}

\end{table}


\subsection{Throughput Evaluation} \label{subsubsec:throughput_eva}
We evaluate the throughout and resource consumption of proposed FPGA implementation of ThundeRiNG, as shown in~\Cref{fig:area_and_throughput}.
\Cref{fig:resource_by_instance}  depicts the resource consumption and the implementation frequency with increasing number of instances.
The results show DSP consumption is oblivious to the number of instances since our state sharing technique enables instances to reuse STU.
The frequency slightly drops down with more (FF + LUT) consumption.
\Cref{fig:throughput_by_instance} shows overall throughput with increasing number of instances, where the blue line is the measured throughput and the dashed grey line is the optimal throughput under frequency of 550MHz.
The observed throughput is near linearly related to the number of instances and can be up to 20.95 Tb/s with 2048 instances.
The gap between the optimal line and the our results is because of the decrement of frequency (from 536MHz to 355MHz).




\subsubsection{Comparison with FPGA-based State-of-the-art Works} \label{subsubsec:fpga_compare}

In \Cref{tab:capacity}, we compare ThundeRiNG with two most related state-of-the-art FPGA-based RNGs~\cite{li2011software,bakiri2017ciprng}.
As their implementations are not public available, we linearly scale up their number of PRNG instances according to the reported resource consumption and total resource on our platform while keeping the same frequency.

The results indicate that ThundeRiNG outperforms them significantly.
ThundeRiNG delivers 17.42$\times$ speedup over MRG32k3a while saving 99\% percentage of DSPs.
Even with assuming Li et al. fully utilized the BRAM resources, ThundeRiNG still delivers 1.37$\times$ speedup.
%, not only the highest throughput but also the least consumption of precious hardware resources.


\begin{figure}[ht!]
     \centering
     \includegraphics[width=1\columnwidth]{figures/resource-crop.pdf}
     \caption{Resources consumption versus number of instances}
     \label{fig:resource_by_instance}
     \vspace{-5mm}
\end{figure}

\begin{figure}[ht!]
     \centering
     \includegraphics[width=1\columnwidth]{figures/throughput-crop.pdf}
     \caption{Throughput versus number of instances}
     \label{fig:throughput_by_instance}
     \vspace{-5mm}
\end{figure}

\begin{comment}
\begin{figure}[ht!]
    \centering
    %\hline
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        %\smallskip
        \includegraphics[width=1\linewidth]{figures/resource-crop.pdf}
        \caption{Resources consumption} %{Light Unit}
        \label{fig:resource_by_instance}
    \end{subfigure}
    \smallskip
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/throughput-crop.pdf}
        \caption{Throughput}
        \label{fig:throughput_by_instance}
    \end{subfigure}
%\hline
    \caption{The area efficiency and throughput with different number of instances}
    \label{fig:area_and_throughput}
    \vspace{-4mm}
\end{figure}
\end{comment}

\begin{table}[ht!]
\caption{The comparison of capacity with FPGA-based work on U250 platform}
\label{tab:capacity}
\resizebox{0.476\textwidth}{!}{%
\begin{tabularx}{0.65\textwidth}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Algorithms}}
& \multirow{2}{*}{\textbf{Freq}}
& \multirow{1}{*}{\textbf{Max}}
& \multirow{2}{*}{\textbf{BRAMs}}
& \multirow{2}{*}{\textbf{DSPs}}
& \multirow{1}{*}{\textbf{LUT + FF}}
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Throughput}}}
\\

&&\multirow{1}{*}{\textbf{\#ins.}}
&
&
&\multirow{1}{*}{\textbf{per ins.}}
&\multirow{1}{*}{\textbf{(Tb/s)}}
&\multirow{1}{*}{\textbf{Ours Sp.}}
\\ \midrule

 \textbf{ThundeRiNG}                             &  \textbf{355} &  \textbf{2048}  &   \textbf{0\%}  &   \textbf{1\%}  &  \textbf{596} & \textbf{20.9}   & \textbf{1}  \\
Li et al.~\cite{li2011software}        & 475 & 1000  & 100\% &  0\%  & 643 & 15.2  & 1.37   \\
MRG32k3a~\cite{bakiri2017ciprng}       & 175 & 1534  &  0\%  & 100\% & 2414 &  1.2 & 17.42  \\
\bottomrule

\end{tabularx}%
}

\end{table}



\subsubsection{Comparison with Existing Works on GPU}

%~\Cref{tab:gpu_througput} shows that ThundeRiNG outperforms the state-of-the-art implementations on Nvidia Tesla P100 GPU platforms from 10.6x to 24.92x. We benchmark the throughput of cuRAND library following the performance optimization guide in~\cite{cuRANDguide}, and we obtain the BigCrush result (second column in~\Cref{tab:gpu_througput}) from the same document.

%~\Cref{tab:gpu_througput} shows the throughput comparison between ThundeRiNG and the cuRAND library which is implemented on a Nvidia Tesla P100 GPU.
%cuRAND library is the official GPU based RNGs from Nvidia. state-of-the-art GPU implementations

%We benchmark the throughput of cuRAND library following the performance optimization guide in~\cite{cuRANDguide} and obtain the BigCrush results from the same document.
We implement the official GPU based RNGs from Nvidia (cuRAND library) on a Nvidia Tesla P100 GPU and compare its throughput with ThundeRiNG, as shown in ~\Cref{tab:gpu_througput}.
In addition, the  BigCrush results are collected from the official document~\cite{cuRANDguide}.

The results show the ThundeRiNG outperforming GPU-based solutions from 10.6$\times$ to 24.92$\times$. It is noteworthy that only two of the GPU-based RNGs pass the BigCrush testing.


\begin{table}[t!]
\caption{Throughput (GSample/s) of various GPU PRNG schemes running on Nvidia Tesla P100 compared to ThundeRiNG's FPGA throughput of 654.53~GSample/s.}
\label{tab:gpu_througput}
\resizebox{0.476\textwidth}{!}{%
\begin{tabularx}{0.65\textwidth}{lccc}
\toprule
\multirow{1}{*}{\textbf{Algorithms in cuRAND}}
& \multirow{1}{*}{\textbf{BigCrush}}
& \multirow{1}{*}{\textbf{Throughput}}
& \multirow{1}{*}{\textbf{ThundeRiNG's Speedup}} \\

%\multirow{1}{*}{\textbf{ }}
%& \multirow{1}{*}{\textbf{}}
%& \multirow{1}{*}{\textbf{ }}
%& \multirow{1}{*}{\textbf{Speedup}} \\

\midrule
Philox-4×32       & 0 &   61.6234 &   $\bm{10.62\times}$     \\
MT19937           & 0 &   51.7373 &   $12.65\times$          \\
MRG32k3a          & 1 &   26.2662 &   $\bm{24.92\times}$     \\
xorwow            & 1 &   56.6053 &   $11.56\times$          \\
MTGP32            & 1 &   29.1273 &   $22.47\times$          \\
\bottomrule


\end{tabularx}%
}

\end{table}


\subsection{Applications}

To further demonstrate the advantages of ThundeRiNG, we apply it to two practical applications with the architecture described in~\Cref{fig:architecture_overview}.
The first application is the estimation of $\pi$. %of which basic principle is that randomly generating two-dimensional points in the unit square then counting the number of points in the unit circle.
The second application is Monte Carlo option calculation for Black-Scholes model, one of the widely used real option analysis method.
Both of the GPU implementations use Philox-4×32 PRNG, which is proven to be the fastest PRNG on GPU.


\Cref{tab:gpu_application} shows the comparison between FPGA and GPU.
The power efficiency is calculated by the throughput divided by run-time power consumption. The measurement of power consumption is taken by the official tools (GPU: nvidia-smi, FPGA: xbutil).
Firstly, our method achieved 8.96$\times$ and 2.55$\times$ speedup in the end-to-end throughput.
The throughput of FPGA-based implementation is very close to the throughput of PRNG, that is because the application processing can be fully pipelined with the generation of random numbers, which is not achievable in GPU platform.
Secondly, ThundeRiNG demonstrate at least 8$\times$ improvement on power efficiency compared to GPU-based implementations, showing PFGA is an attractive platform for PRNG related applications.

\begin{table}[t!]
\caption{The comparison of throughput and power efficiency on real applications}
\label{tab:gpu_application}
\resizebox{0.476\textwidth}{!}{%

\begin{tabularx}{0.67\textwidth}{llcc}
\toprule

\multicolumn{2}{l}{\multirow{1}{*}{\textbf{Applications}}}
& \multirow{1}{*}{\textbf{Estimation of $\bm{ \pi }$}}
& \multirow{1}{*}{\textbf{MC Black Scholes }} \\\midrule


\multicolumn{2}{l}{\multirow{1}{*}{Number of draws}} & $3\times10^{11}$ & $3\times10^{11}$ \\ \hline
\\[-1em]

& Frequency (MHz) & 304      &  335 \\
& Number of instances  & 1600 &  256  \\

\multicolumn{1}{c}{\multirow{3}{*}{ FPGA: Alveo U250 }}
& LUTs    & 1048235(70\%)  &  735173(49\%)    \\

\multicolumn{1}{c}{\multirow{3}{*}{ (16nm FinFET) }}
& FFs     & 1171130(38\%)  &   751810(24\%)   \\
& DSPs    & 5512(45\%)     &   5984(49\%)      \\
\cmidrule(lr){2-4}
&Execution time (s) & 1.248 & 3.499          \\
&Throughput (GSample/s) & 480 & 86  \\
&Power consumption (W) & 45  & 43 \\ \hline
%-----------------------------------------------------------------------
\\[-1em]
\multicolumn{1}{c}{\multirow{2}{*}[-0.5em]{GPU: Tesla P100 } }
& Frequency (MHz) & 1,190  &  1,190 \\
\cmidrule(lr){2-4}

\multicolumn{1}{c}{\multirow{2}{*}{ (16nm FinFET) }}
&Execution time (s)  & 11.190 & 8.908 \\
&Throughput (GSample/s) & 53 & 33 \\
&Power consumption (W) & 131  & 126 \\  \hline
\\[-1em]

\multirow{1}{*}{ThundeRiNG's }
& Throughput Speedup& \textbf{8.96x}  &  \textbf{2.55x} \\

\multirow{1}{*}{Improvement }
& Power efficiency & \textbf{26.10x} & \textbf{7.46x} \\\bottomrule


%49




%%& \multicolumn{3}{c}{\multirow{1}{*}{\textbf{Execution time (s)}}}
%& \multicolumn{3}{c}{\multirow{1}{*}{\textbf{Performance/Energy (GSample/W)}}} \\
%
%
%&
%&\multirow{1}{*}{\textbf{P100}} & \multirow{1}{*}{\textbf{Ours}} & \multirow{1}{*}{\textbf{Speedup}}
%&\multirow{1}{*}{\textbf{P100}} & \multirow{1}{*}{\textbf{Ours}} & \multirow{1}{*}{\textbf{Speedup}}\\
%
%Estimatie PI               &  $3\times10^11$ &   37.69 &   1.63 & 23.15
%& \\
% &   &   449.79  &   7.95\\ \bottomrule

\end{tabularx}%
}

\end{table}






==> commented/5.5-related_work.tex <==

\section{Related Work}\label{sec:related_work}

\todo[inline]{I don't think we need this related work section anymore. Just try to simply insert the contents here into the intro and background.}

There are a few existing working on exploring PRNG on FPGAs.
To the best of our knowledge, there is only one work from Li et al. ~\cite{li2011software} that considers the generation of multiple independent random number sequences with enough degree of parallelism.
They adopt the commonly used jump-ahead method for a WELL based generator and provide the analysis of inter-stream correlation.
However, their crush testing falls short in two failures, and the consumption of BRAMs limits the number of independent generators on FPGA platform.
Binary linear generators can be efficiently implemented on FPGA platforms but support a limited degree of parallelism for the generation of multiple sequences~\cite{thomas2012lut,dalal2008fast}.
% first work
Dalal et al.~\cite{dalal2008fast} map the existing Mersenne Twister algorithm into FPGA platform. %The large bit width of state leads to the requirement of Block RAM (BRAM) to store it.
The generation of multiple sequences is based on the direct partition of the state; hence, the maximum degree of parallelism is limited by the width of state.
According to the PRNG used in their paper, the WELL44497 generator, whose the the state is 44497-bit width, can only support 107 distinct streams.'
They use the WELL44497 generator with  44497-bit state, which supports only 107 distinct streams.
% second work
LUT-SR~\cite{thomas2012lut} is a resource efficient PRNG on FPGAs and highly optimized for shift register LUTs. It supports a large-bit (up to 19937) state transition without the cost of BRAMs.
However, as the algorithm is based on the linear recurrence, which have flaws on the linear complexity, LUT-SR is not crush-resistant and lacks the support of generating multiple sequences.
%
%Dalal et al.~\cite{dabal2014study} proposes a chaotic PRNG


% The stage of PRNG which comparatively demands more computation (multiplicaton takes greater weight compared to bit-wise operations);
% Which type of hardware resources is excessively consumed (the consumption is accounted by the percentage over available resources).

%Bakiri, et al.~\cite{bakiri2017ciprng} also evaluate the existing crush-resistant algorithms: MRG32k3a~\cite{l1999good}, PCG\_XSH\_RS\_64~\cite{o2014pcg} and xorshift64*~\cite{marsaglia2003xorshift} on FPGA platform. MRG32k3a~\cite{l1996combined} is a well-known PRNG and has been implemented both in Intel MKL and Nvidia cuRAND libraries. It combines two LCGs of which the modulus is not a power of 2, hence the modulo operations need an additional divider which is very resource costly. PCG\_XSH\_RS\_64~\cite{o2014pcg} invokes a random rotation permutation over LCG to improve the statistical quality, and it needs a large bit multiplication during the state transition. xorshift64*~\cite{marsaglia2003xorshift} adopts a invertible multiplication on the output of xorshift as a nonlinear transformation to enhance the quality. All of the three PRNGs support the jump-ahead technique for generating multiple independent streams. Despite the high quality and capability of multiple sequence generation, these algorithms also involve multiplication arithmetics which lead to large consumption of DSP slices.






==> commented/background-legacy.tex <==
%!TEX root = main.tex

\section{Background and Related Work}\label{sec:background}
\newenvironment{conditions}
  {\par\vspace{\abovedisplayskip}\noindent\begin{tabular}{>{$}l<{$} @{${},{}$} l}}
  {\end{tabular}\par\vspace{\belowdisplayskip}}

% \todo[inline]{[DONE] Can split the background and related work into 2 sections. Currently they are not strongly connected and a single section should not contain too much info.}
In this section, we introduce the statistical randomness concept as well as the testing method for systemic evaluating of a PRNG, followed by the review of existing methods for multiple sequence generation. Furthermore, a brief introduction of LCG is presented as the background for the depiction of ThunderRiNG.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Statistical Randomness and Empirical Testing }\label{subsec:randomness_test}
%Now that we have a glimpse of how to generate random numbers, we can look at ways to judge whether a PRNG is good or not.
% the ability to skip ahead or jump back a certain number of elements in the sequence produced
%Speed, period, repeatability and seekability (the ability to skip ahead or jump back a certain number of elements in the sequence produced) are four important indicators of the quality of PRNGs. and
\subsubsection {Statistical randomness}
The most important indicator of the quality of PRNGs is the randomness for successive output values to behave as independent, identically distribution (i.i.d) random variables. However, randomness is hard to measure, instead, statistical randomness is commonly used for the judgment of a PRNG. Typically, a numeric sequence is statistically random when it contains no recognizable pattern or regularities~\cite{wiki:sr}.

The most important indicator of the quality of PRNGs is the randomness, which indicates the independence, identically distribution (i.i.d) random variables.
However, true randomness is hard to measure (why it is hard); instead, statistical randomness is commonly used for the judgment of a PRNG.
A numeric sequence is statistically random when it contains no recognizable pattern or regularities~\cite{wiki:sr}.


\subsubsection {Evaluation of statistical randomness}
There are a lot of different testing approaches for the statistical randomness of a PRNG. These tests can be categorized into two groups: theoretical testings and empirical testings. Theoretical test is a kind of prior tests based on the knowledge of the PRNG structure and it is not sufficient in many cases~\cite{10.5555/270146}. Empirical tests are more widely used to tell a PRNG is good or not, it is conducted on a generated sequence and require no knowledge of how the PRNG produces the sequence. These tests rely on the null hypothesis testing of the statistic properties of input sequences with the assumption of i.i.d.


\subsubsection {Empirical testing}
Several systematic empirical test suites for PRNGs~\cite{marsaglia1995diehard,bassham2010sp,brown1994security} are proposed. The most complete and stringent test is TestU01~\cite{l2007testu01} which provides a consistent framework as well as batteries of tests that are supersets of the earlier suites, in addition to an assortment of tests from other sources that had not previously been incorporated into a battery. The predefined batteries in TestU01 include SmallCrush (10 tests), Crush (96 tests) and BigCrush (160 tests). PRNGs that pass all tests in those batteries can be referred as \textbf{\textit{crush-resistant}} while the PRNGs failed to pass is \textbf{\textit{crushable}}~\cite{salmon2011parallel}. Note that, A crush-resistant PRNG can never prove it is flawless, but if there are failed tests, it definitively indicates that there are known patterns existing in this generation algorithm which should be carefully considered in applications.
% it is ambiguous and lacks deterministic guideline, More importantly,

\subsection{Multiple Sequence Generation}\label{subsec:multiple_sequences_generation}
%\subsubsection {Degree of parallelism}
Generating multiple sequences is a common parallelization method to improve the throughput of the PRNGs.
%Parallelizing the generation of random sequences is not completely new,
In summary, there are two different strategies, but all of them have practical limitations.

\noindent
\textbf{Substream.}
(1) for the PRNG with good seekability and long period, it can be divided into many disjoint \textbf{\textit{substreams}} by using fast jump ahead technique~\cite{haramoto2008efficient} which can determine the starting position of the new substream efficiently. De Matteis et al.~\cite{de1992computation} points out that substreams still have potential long-range correlations in certain cases;


\noindent
\textbf{Multistream.}
(2) different instances of a generation algorithm with very large output space but hard to jump ahead can be seeded differently by the assumption of a very low probability of overlapping among the sequences. However, this overlapping probability increases dramatically following to growth of the number of instances. Thus, this method needs a well-tuned and carefully verified seed initialization mechanism which is always ignored by existing work. Samuel et al.~\cite{neves2011fast} only consider the probability of collisions while ignores the probability of the correlation introduced by an adjacent or near state.
(3) independent generators of the same family are configured using different algorithmic parameters such as the multipliers or shifts. This approach is also referred as \textbf{\textit{multistreams}}, the problem of this approach is that, the parameters are enumerable from a finite set which has a comparatively small and limited space. More importantly, this method is also proved to be elusive to emulate all possible parameters~\cite{salmon2011parallel}. We use \textbf{\textit{degree of parallelism}} referred to the number of instanced independent generators. the maximum degree of parallelism for a PRNG algorithm is deterministic.

\subsection {Inter-stream and intra-stream correlation} \label{subsec:inter-stream}
Despite there are many existing test suites for PRNGs, they are all focus on the testing of dependencies on single sequence (\textbf{\textit{intra-stream}}) while the dependencies between multiple sequences (\textbf{\textit{inter-stream}}) are overlooked in many testing suits.
TestU01~\cite{l2007testu01} deploys two basic schemes for testing the inter-stream correlation: two-level tests and parallel filter. However, both of the above methods fail to recognize the multivariate nature of the dependency in parallel generation. The two-level tests apply serial tests to the individual streams and then combine the statistics of each testing based on their distribution. The problem is that the serial testing of single stream, which is based on the null hypothesis, loses the information of the original data by reducing each vector to a single statistical measurement. Therefore, the aggregation of these measurement is necessary but far away from sufficient to indicate the independence of inter-stream. The parallel filter combines all the parallel generated streams into a long stream, in which each stream stacks on the top of the previous one, and then applies serial tests to the resulting concatenated stream. It can be failed to detect the correlation of a very closed correlation of two distinct streams which can be far away from each other in the flattened one-dimensional sequence because of the stacking concatenation.

Existing works verify the inter-stream correlation in different ways.~\cite{salmon2011parallel} introduced a specific testing method which is only usable for the counter-based generator.  Li, et al.~\cite{li2011software} tests the inter-stream correlation by interleaving the substreams into one single sequence then applying the TestU01 on the new sequence to obtain a systematic evaluation of the inter-stream correlation. This approach avoids the two problems we mentioned above: There is no loss of information in the data, and it combines streams in the way that is same to the pattern when the random numbers are consumed. We adopt this interleaving test as the systemic evaluation of the dependency among multiple sequences. In addition to it, we also conduct the two additional tests to demonstrate the effectiveness of our decorrelation approach. We first analyze cross-correlation of different streams and then conduct the testing of Hamming weight dependencies following the~\cite{blackman2018scrambled} to further analysis the inter-stream Hamming weight dependencies (statistical bias in the number of zeros and ones in each output) which is the potential dependency brought by the sharing of state. The details is available in~\Cref{subsubsec:details}.
\subsection{Related Work}\label{sec:related_work}

%\subsection{Methods for Multiple Sequences Generation}\label{sec:sub_parallel_methods}


%The existing parallel methods can be summarized as two classes: substream and multstream, but both approaches have practical limitations.
%In substream methods, a viable generator with very long period is divided into many disjoint substreams by using fast jump ahead technique.

%However it usually requires large state space and . For the multistream approach, the PRNG algorithm is instantiated in parallel with different parameters, these parameters are only finite enumerable sets which proven elusive and have scalability problem
In~\Cref{tab:cost_prng}, we summary the state-of-the-art works.~\cite{thomas2012lut,dalal2008fast,li2011software} are all binary linear generators which can be efficiently implemented on FPGA platform.~\cite{thomas2012lut} propose a shift register LUT (SRL)
based generator which is most resource efficient over all of the other generators. However, it is not crush-resistant and lacks the support of the generation of multiple sequences and the corresponding correlation analysis. More importantly, the parameters for the distinct generators are also limited.~\cite{dalal2008fast} mapping the existing Mersenne Twister algorithm into FPGA platform. The large bit width of state leads to the requirement of Block RAM (BRAM) to store it. The generation of multiple sequences is based on the partition of state, and the maximum degree of parallelism is limited by the bit width of state: for a WELL44497 generator, it only support 107 distinct streams which is comparative small.~\cite{li2011software} adopt the commonly used jump ahead method for a WELL-based generator on the FPGA platform, and they also provide the analysis of inter-stream correlation. However, it has two failures on the crush testing, and the consumption of BRAMs also limits the capacity of independent generators on hardware.

Bakiri, et al.~\cite{bakiri2017ciprng} also evaluate the existing crush-resistant algorithms: MRG32k3a~\cite{l1999good}, PCG\_XSH\_RS\_64~\cite{o2014pcg} and xorshift64*~\cite{marsaglia2003xorshift} on FPGA platform. MRG32k3a~\cite{l1996combined} is a well-known PRNG and has been implemented both in Intel MKL and Nvidia cuRAND library. It combines two LCGs of which the modulus is not a power of 2, hence the modulo operations need additional divider which is very resource costly. PCG\_XSH\_RS\_64~\cite{o2014pcg} invokes a random rotation permutation over LCG to improve the statistical quality, and it needs a large bit multiplication during the state transition. xorshift64*~\cite{marsaglia2003xorshift} adopts a invertible multiplication to the output of xorshift as a non-linear transformation to enhance the quality. All of the three PRNGs support the jump ahead technique for generate multiple independent streams. Despite the high quality and the ability of multiple sequences generation, these algorithms also involve multiplication arithmetics which lead to large consumption of DSP slices.



%There are some existing crush-resistant parallel RNGs on CPU and GPU. . Salmon et al.~\cite{salmon2011parallel} proposed a counter-based PRNG named Philox that can generate $2^{64}$ unique parallel streams. Recently, Blackman et al.~\cite{blackman2018scrambled} developed a new scrambler which based on filtered linear-feedback shift register theory for existing generators, and this generation algorithm also has fast jump ahead mechanism enabling the substream parallelization.

%According to this survey~\cite{bakiri2018survey} in 2018, there is even no existing crush-resistant linear PRNG on FPGA and nearly all of them have poor scalability for multiple sequence generation. Li et al.~\cite{li2013software} deployed the jump-ahead mechanism on FPGA along with WELL algorithm, but this method have 2 crush failed. Furthermore, the resource consumption is also a big consideration when design or select PRNG on FPGAs, because the logic resources is not only used by the generator but also the application processing. LUT-SR~\cite{thomas2012lut} is the most resource friendly  method with out using BRAMs, but it is not crush-resistant. Bakiri et al.~\cite{bakiri2017ciprng} evaluated some crush-resistant parallelizable RNGs on FPGAs, such as MRG32k3a, PCG32, xorshift64*, these generators require DSP slices or BRAMs, However, directly applying the existing parallel generation methods also need independent instances of the generator, and it leads to a proportional growth of the consumption of these precious hardware resources with the degree of parallelism. Finally, it become a bottleneck to increase the parallelism especially when the application processing modules also need DSPs or BRAMs.

%From~\Cref{tab:cost_prng}, we can see the most complex part of nearly all PRNGs is the state transition function, and it motivates us to find a way to reduce the cost by sharing the state among different instances. It is obvious that PRNG with large bit state such as MT19937 can not be shared as it can lead to very large overhead of the sharing process. As LCG is well studied in theory, the flaws are known clearly and there are also some existing work which fix these flaws in LCG. Meanwhile, we found that there is a good property in LCG to enable the sharing of the state more easily. Therefore we choice LCG as the base generator in our proposed multiple random sequences generation method.




%or the generated sub-sequences have high correlation or hamming weight dependency which is not acceptable in statistical tests.
%A long period by itself certainly does insure good statistical randomness however is not sufficient to ensure lack of defects.
%Statistical randomness does not necessarily imply "true" randomness, objective unpredictability. Pseudorandomness is sufficient for many uses, such as statistics, hence the name statistical randomness.
%In the common parlance, randomness is the apparent lack of pattern or predictability in events
%The abstract mathematical requirement of an PRNG is that it can produce an i.i.d.(independent and identically distributed) sequence and
%
%Producing an independent and identically distributed sequence


%It is obvious that the sequence generated by PRNG is not true randomness as it is deterministic or predictable.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Linear Congruential Generator}\label{subsec:lcg}
%Our method is based on the linear congruential generator (LCG), one of the oldest algorithms for generating pseudo-randomized numbers.
%\todo[inline]{[DONE] Is there any design specific information in this subsection?--> yes, if not, this should be introduced in the background rather than the method.}

The linear congruential generator (LCG) $X_{a,m}^c$ is defined by the following recurrence relation~\cite{10.5555/270146}:

\begin{equation}
 x_{n+1} = a \cdot x_{n} + c \pmod{ m }, ~~n \geq 0 \label{eq:lcg}
\end{equation}
\noindent \textit{Where:}
\begin{conditions}
~m     & the \textbf{\textit{modulus}}, $m \in \mathbb{Z}^{+} $. \\
~a     & the \textbf{\textit{multiplier}}, $0 < a < m$.          \\
~c     & the \textbf{\textit{increment}}, $0 \leq c < m$.        \\
\end{conditions}

%The period of LCG, $p$, . The period is an important property of a generation algorithm, and it should be much longer than any sequence that will be used in any application.


LCG is well-studied in theory. If $c = 0$, the generator is often called a multiplicative congruential generator (MCG). When  $c\neq0$, the new sequence can be  affine transformed from the MCG~\cite{steele2020computationally}, and the selection of $a$ and $c$ should follow the Hull-Dobell Theorems~\cite{hull1962random} to maximize the period, which is defined as the smallest integer to hold the equation $x_{n+p}=x_{n}$ for all $n$.~\Cref{eq:lcg} can be treated as the state transition function, and it always conducts the bit truncation on $x_{n}$ in the output stage to make sure the state space is larger than output space (requirement of birthday paradox). LCG has been evaluated that most flaws of it come from a small state space~\cite{o2014pcg}, and its lower bits is also known to have a shorter period. Therefore, there are many existing algorithms~\cite{o2014pcg,l1996combined} focus on solving these problems.

%Note that, despite the distinct sequences can be generated by selecting different $c$ easily, it has been already known that these sequences are not statistically independent from each other: they are highly correlated, and the difference of corresponding Hamming weight can be very small.

LCGs can leverage the generation of multiple sequences by either multistreams and substreams approach. The substreams method, which splits the space of state, requires independent generators and results in proportional requirement of resources.
%Due to this reason we do not consider it as the candidate for state sharing.??????
For multistreams method, there are two different approaches: the first one is that each LCG is assigned with different multiplier and the same modulus, while the second approach focus on the modulus: for each different LCG, it will have a distinct modulus and an optimal multiplier. It has been evaluated that the parameter set for both two methods are very limited and hard to emulate all of the valid parameters because it involves the primality testing for large numbers.

LCGs with same modulus and multiplier but different increments can also generate distinct sequences, and the total number of distinct sequences can be very large. For example, if we choose the modulus as $2^{64}$, according to the Hull-Dobell Theorems~\cite{hull1962random}, the increment should be odd to guarantee that each generator is full cycle. Therefore, the number of distinct sequences can be up-to $2^{63}$ which is large enough for parallel processing. ~\cite{durst1989using} indicates that these sequences are proven to be highly correlated with each other. However, such approach (we call it parameterization via increment) can also provide large degree of parallelism if the correlation is well handled.

We adopt a lightweight decorrelator to handle the above correlation. Furthermore, we find a mechanism that can generate distinct any number of distinct sequences without the increasing of multiplication arithmetic which is resources efficient on FPGA architectures. Combining these two processes together, we enable the concurrent generation of massive high quality random numbers. To give an intuitive illustration of our method, the following definition of LCG set, which is a set all of the LCGs parameterized via increment, is provided:
\theoremstyle{definition}
\begin{definition}[LCG set]{}
A set of sequences generated by LCGs with the same $a$, $m$ and distinct $c$ is defined as $\mathbb{X}_{a,m} = \lbrace X_{a,m}^{c}, \: ...\mid{}  {0 \leqslant c < m}  \rbrace$.
There is only one multiplicative congruential generator (MCG) ${X'}_{a,m}$ (when~$c = 0$) in $\mathbb{X}_{a,m}$,
and any element in $\mathbb{X}_{a,m}$ can be transformed from ${{X'}_{a,m}}$ by the corresponding affine transformation function: $X_{a,m}^{c}=\varphi_c({X'}_{a,m}), where ~ \varphi_c \colon U \to U $ ($U$ is the output space).
\end{definition}





% LCG has been well-studied in theory. It has been evaluated that most flaws of LCGs come from a small state space, and there is a crush-resistant LCG which have %96-bit state.
%Moreover, some applications need very large period resulting a larger bit-width of state.
%However, the multiplication of 96-bit or larger state can be very inefficient on modern hardware.
%Specifically, CPU or GPU need to split the value into smaller chunk and recombine the output of multiplication calculation,
%while FPGA can be more flexible in such case because it can directly build any bit multiplier by the logic resources,
%but the consumption of hardware resources is linear related with the number of instances,
%it seems optimal while still can not be acceptable if there is a high requirement of the degree of parallelism with a limitation %of hardware resources.

%Therefore, our goal is to find a way to reduce resource consumption, by ~\Cref{thm:state_sharing}, we know that the new sequence $Y$ which is distinct but have the same statistics quality with the original


==> commented/commented.tex <==
%\subsubsection{Evaluation Outline} \label{evaluation_outline}


\subsection{The Selection of LCG and Decorrelator} \label{subsubsec:selection_of_decorr}

\begin{table}[h!]
\caption{The comparison of different decorrelator}
\label{tab:selection_of_decorr}
\resizebox{0.476\textwidth}{!}{%
\begin{tabularx}{0.6\textwidth}{lcccc}
\toprule

\multicolumn{3}{c}{\multirow{1}{*}{\textbf{Decorrelator}}}
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Maximum degree of parallelism}}}
\\ \cline{1-3}

\multirow{2}{*}{\textbf{Algorithms}}
& \multirow{1}{*}{\textbf{Systematic}}
& \multirow{1}{*}{\textbf{Resources}}
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{(Crush-resistant)}}}
\\ \cline{4-5}


& \multirow{1}{*}{\textbf{Failures}}
& \multirow{1}{*}{\textbf{(LUT + FF)}}
& \multirow{1}{*}{\textbf{Theoretical}}
& \multirow{1}{*}{\textbf{Evaluated}}
\\
\midrule

xorshift32      & 75  &  275   &  1             &     $2^{12}$       \\
xorshift64      & 32  &  563   &  1             &     $2^{16}$       \\
xorshift128     & 7   &  1125  &  $2^{64}$      &    up to $2^{32}$  \\
xorwow          & 20  &  2076  &  $2^{128}-1$   &    up to $2^{32}$  \\
\bottomrule

\end{tabularx}%
}

\end{table}
























\begin{comments}
%Based on the results in \Cref{tab:correlation_results}, we have the following observations.
 LCG (parameterization via increment but without decorrelation) has high correlation and fails on almost all of the testings in BigCrush.
After applying the decorrelation method, there is a significant improvement on the independence: Firstly, the cross-correlation decreases from 0.97 to 0.0046 which is very close to zero. Secondly, there is no sign of Hamming weight bias after generating 100 trillions of random number while the original one fails before 125 millions.
As a result, there are only 4 failures in BigCrush testing. The results of ThundeRiNG which concludes the decorrelation and permutation are shown in the fourth row, it shows that the permutation makes the quality better.

We also perform the tests on the LCG with permutation to validate that the improvement of independence is only come from our decorrelation approach. The results show that permutation also reduces the cross-correlation, but there is no improvement on Hamming weight dependence. The reason is that permutation introduces non-linearity in the sequence which reduce the similarity significantly, but as a bijective remapping, it dose not change the Hamming weight, therefore the bias of Hamming weight is reserved.
\end{comments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%


We further evaluate the strength of our proposed decorrelation method by applying the cross-correlation analysis (a measure of similarity of two sequences) and Hamming weight dependency testing.
Firstly, the cross-correlation is measured by iteratively calculating it between two randomly selected distinct sequences and reporting the maximal number over 1000 times testings.
If the streams are independent with each other, the cross-correlation should be close to zero.
Secondly, as the state which has the same Hamming weight is reused among many instances, there is potential statistical bias in the Hamming weight of the different sequences.
Therefore we apply the latest Hamming weight dependency(HWD) testing from~\cite{blackman2018scrambled}, which can discover more bias patterns of HWD than the BigCrush. The result from this HWD testing indicates the number of generated random numbers before an unexpected pattern is detected, hence, higher value is better.
Finally, the BigCrush for multiple sequences is also performed for each method.
%We conduct four testings to evaluate the statistical quality of ThundeRiNG.
\begin{comment}

We conduct four statistical testings on ThundeRiNG and state-of-the-art RNG algorithms,
Firstly, the statistical properties of single sequence is evaluated under the BigCrush battery~\cite{l2007testu01} from TestU01 suite.
The number presented in the second column indicates the number of failures.
Then we follow the interleaving method in ~\cite{li2011software} to check the correlation between different sequences, rather than the original method that only uses the Crush battery, we apply BigCrush on the interleaved stream.
Thirdly, we calculate the maximum cross correlation in a set of randomly selected streams.
Finally, we follow the latest HWD testing method~\cite{blackman2018scrambled} whose result indicates the number of generated random numbers before an unexpected pattern occurs (higher is better).
The HWD test is applied on the same interleaved stream as the second test to further verify the independence of distinct sequences.
We evaluate Statistical Quality under the

\subsubsection{Benefits of decorrelation and permutation}.
We evaluate decorrelation and permutation in terms of Cross-correlation and HWD
We incrementally enable decorrelation and permutation methods on LCG to demonstrate the corresponding improvements on the independence among multiple sequences, as shown in \Cref{tab:correlation_results}.
%Three correlation tests are conducted as shown in .
Cross-correlation is calculated by two randomly selected distinct sequences and reported with the maximal number over 1000 times testings.
HWD is another dependence metric and commonly adopted for empirical testing.  It is measured with the latest HWD testing method~\cite{blackman2018scrambled}, and the value indicates the number of generated random numbers before an unexpected pattern occurs (higher is better).
The HWD test is applied on the same interleaved stream as the second test to further verify the independence of distinct sequences.

%Firstly, to calculate the cross-correlation, two distinct sequences are randomly selected. we repeat this random process up to 1000 times to get the maximum cross-correlation.
%We show the maximum cross-correlation over 1000 times processes in the table.



%To show the approach's improvement on the Hamming weight dependence (HWD


%decorrelator improves the HMD over the orginal LCG. However,  only with it, it still has
Although enabling decorrelator to LCG improves the HMD, there still remains a fail. in ....since .....
this problem is not .....


The effectiveness of decorrelator is shown in the third row. Comparing with the original LCG (in the second row), our decorrelation method significantly reduces the cross correlation from 0.97 to 0.046, and the HWD testing result of decorrelation indicates there is no sign of bias even after 400 Tbytes of output.
However, it has some failures in the BigCrush, but these failures are eliminated in the ThundeRiNG by adopting the additional permutation.
We also test the multistream dependence of PCG32-XSH-RR~\cite{o2014pcg} of which the permutation is used by ThundeRiNG. The results show that the correlation is very small, but the HWD testing result is bad. This is because that the permutation introduces non-linear relation between different sequences, but, as a bijection function, it does not change the Hamming weight; hence, it also has many failures in BigCrush of multiple sequences.
\end{comment}



%\subsubsection{Sequential Testing}
%The BigCrush is used in this experiment. We first evaluate the statistical quality of many single sequences by randomly selecting the stream initialization tuple ($h$, $S_k$) and then feed the generated sequences to test battery independently. Overall, we select up to 100 exclusive configurations, which result in 16000 tests, and our method is succeed to pass all the tests.


%\subsubsection{Multi-sequences Testing } \label{subsubsec:correlation_results}

%We test the correlation and dependency of multiple sequences by three testings. Firstly, we select the sequences with adjacent ($h$, $S_k$) and calculate the cross correlation $\rho$ in  and then we choose up to 4096 sequences and interleave them into a single stream, and apply the new stream to the BigCrush battery~\cite{li2011software}. Finally, we test the Hamming weight dependency (HWD) on above interleaved sequence by the latest testing method proposed in~\cite{blackman2018scrambled}, the HWD testing exact the regular pattern in a successive way, therefore, a litte number means such pattern is detected very early which is considered to be bad (higher is better).
% the third column




@inproceedings{kapre2017applying,
  title={Applying models of computation to opencl pipes for fpga computing},
  author={N. Kapre et al.},
  booktitle={IWOCL},
  year={2017}
}

@article{hellekalek1998good,
  title={Good random number generators are (not so) easy to find},
  author={P. Hellekalek},
  journal={Mathematics and Computers in Simulation},
  volume={46},
  number={5-6},
  pages={485--505},
  year={1998},
  publisher={Elsevier}
}

@article{haramoto2008efficient,
  title={Efficient Jump Ahead for F2-Linear Random Number Generators},
  author={Haramoto, Hiroshi and Matsumoto, Makoto and Nishimura, Takuji and Panneton, Fran{\c{c}}ois and L'Ecuyer, Pierre},
  journal={INFORMS Journal on Computing},
  volume={20},
  number={3},
  pages={385--390},
  year={2008},
  publisher={INFORMS}
}

@article{de1992computation,
  title={Computation of critical distances within multiplicative congruential pseudorandom number sequences},
  author={De Matteis, Artenio and Eichenauer-Herrmann, J{\"u}rgen and Grothe, Holger},
  journal={Journal of Computational and Applied Mathematics},
  volume={39},
  number={1},
  pages={49--55},
  year={1992},
  publisher={Elsevier}
}

@inproceedings{salmon2011parallel,
  title={Parallel random numbers: as easy as 1, 2, 3},
  author={Salmon, John K and Moraes, Mark A and Dror, Ron O and Shaw, David E},
  booktitle={Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--12},
  year={2011}
}

@inproceedings{thomas2010fpga,
  title={Fpga-optimised uniform random number generators using luts and shift registers},
  author={Thomas, David B and Luk, Wayne},
  booktitle={2010 International Conference on Field Programmable Logic and Applications},
  pages={77--82},
  year={2010},
  organization={IEEE}
}


@inproceedings{li2011software,
  title={Software/hardware framework for generating parallel long-period random numbers using the well method},
  author={Li, Yuan and Chow, Paul and Jiang, Jiang and Zhang, Minxuan},
  booktitle={2011 21st International Conference on Field Programmable Logic and Applications},
  pages={110--115},
  year={2011},
  organization={IEEE}
}

@article{l1999good,
  title={Good parameters and implementations for combined multiple recursive random number generators},
  author={L'ecuyer, Pierre},
  journal={Operations Research},
  volume={47},
  number={1},
  pages={159--164},
  year={1999},
  publisher={INFORMS}
}

@article{o2014pcg,
  title={PCG: A family of simple fast space-efficient statistically good algorithms for random number generation},
  author={O’Neill, Melissa E},
  journal={ACM Transactions on Mathematical Software},
  year={2014}
}

@article{marsaglia2003xorshift,
  title={Xorshift rngs},
  author={Marsaglia, George and others},
  journal={Journal of Statistical Software},
  volume={8},
  number={14},
  pages={1--6},
  year={2003}
}

@INPROCEEDINGS{4616765,
  author={ {JunKyu Lee} and G. D. {Peterson} and R. J. {Harrison} and R. J. {Hinde}},
  booktitle={2008 51st Midwest Symposium on Circuits and Systems},
  title={Hardware accelerated Scalable Parallel Random Number Generators for Monte Carlo methods},
  year={2008},
  volume={},
  number={},
  pages={177-180},
  doi={10.1109/MWSCAS.2008.4616765}}


@article{10.2307/24949798,
 ISSN = {00368733, 19467087},
 URL = {http://www.jstor.org/stable/24949798},
 author = {Gregory J. Chaitin},
 journal = {Scientific American},
 number = {5},
 pages = {47--53},
 publisher = {Scientific American, a division of Nature America, Inc.},
 title = {RANDOMNESS AND MATHEMATICAL PROOF},
 volume = {232},
 year = {1975}
}

@misc{ wiki:sr,
  author = "{Wikipedia contributors}",
  title = "Statistical randomness --- {Wikipedia}{,} The Free Encyclopedia",
  year = "2020",
  url = "https://en.wikipedia.org/w/index.php?title=Statistical_randomness&oldid=948430929",
  note = "[Online; accessed 29-October-2020]"
}

@book{10.5555/270146,
author = {Knuth, Donald E.},
title = {The Art of Computer Programming, Volume 2 (3rd Ed.): Seminumerical Algorithms},
year = {1997},
isbn = {0201896842},
publisher = {Addison-Wesley Longman Publishing Co., Inc.},
address = {USA}
}

@article{marsaglia1995diehard,
  title={The diehard test suite, 1995},
  author={Marsaglia, George},
  journal={URL http://stat. fsu. edu/\~{} geo/diehard. html},
  year={1995}
}

@book{bassham2010sp,
  title={Sp 800-22 rev. 1a. a statistical test suite for random and pseudorandom number generators for cryptographic applications},
  author={Bassham III, Lawrence E and Rukhin, Andrew L and Soto, Juan and Nechvatal, James R and Smid, Miles E and Barker, Elaine B and Leigh, Stefan D and Levenson, Mark and Vangel, Mark and Banks, David L and others},
  year={2010},
  publisher={National Institute of Standards \& Technology}
}


@article{brown1994security,
  title={Security requirements for cryptographic modules},
  author={Brown, Karen H},
  journal={Fed. Inf. Process. Stand. Publ},
  pages={1--53},
  year={1994}
}

@article{l2007testu01,
  title={TestU01: AC library for empirical testing of random number generators},
  author={L'Ecuyer, Pierre and Simard, Richard},
  journal={ACM Transactions on Mathematical Software (TOMS)},
  volume={33},
  number={4},
  pages={1--40},
  year={2007},
  publisher={ACM New York, NY, USA}
}


@article{l1996combined,
  title={Combined multiple recursive random number generators},
  author={L'Ecuyer, Pierre},
  journal={Operations research},
  volume={44},
  number={5},
  pages={816--822},
  year={1996},
  publisher={INFORMS}
}

@article{blackman2018scrambled,
  title={Scrambled linear pseudorandom number generators},
  author={Blackman, David and Vigna, Sebastiano},
  journal={arXiv preprint arXiv:1805.01407},
  year={2018}
}

@article{bakiri2018survey,
  title={Survey on hardware implementation of random number generators on FPGA: Theory and experimental analyses},
  author={Bakiri, Mohammed and Guyeux, Christophe and Couchot, Jean-Fran{\c{c}}ois and Oudjida, Abdelkrim Kamel},
  journal={Computer Science Review},
  volume={27},
  pages={135--153},
  year={2018},
  publisher={Elsevier}
}

@article{li2013software,
  title={Software/Hardware Parallel Long-Period Random Number Generation Framework Based on the WELL Method},
  author={Li, Yuan and Chow, Paul and Jiang, Jiang and Zhang, Minxuan and Wei, Shaojun},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={22},
  number={5},
  pages={1054--1059},
  year={2013},
  publisher={IEEE}
}

@article{thomas2012lut,
  title={The LUT-SR family of uniform random number generators for FPGA architectures},
  author={Thomas, David B and Luk, Wayne},
  journal={IEEE transactions on very large scale integration (vlsi) systems},
  volume={21},
  number={4},
  pages={761--770},
  year={2012},
  publisher={IEEE}
}

@ARTICLE{bakiri2017ciprng,
  author={M. {Bakiri} and J. {Couchot} and C. {Guyeux}},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
  title={CIPRNG: A VLSI Family of Chaotic Iterations Post-Processings for $\mathbb {F}_{2}$ -Linear Pseudorandom Number Generation Based on Zynq MPSoC},
  year={2018},
  volume={65},
  number={5},
  pages={1628-1641},
  doi={10.1109/TCSI.2017.2754650}
}

@article{hull1962random,
  title={Random number generators},
  author={Hull, Thomas E and Dobell, Alan R},
  journal={SIAM review},
  volume={4},
  number={3},
  pages={230--254},
  year={1962},
  publisher={SIAM}
}

@inproceedings{yao1982theory,
  title={Theory and application of trapdoor functions},
  author={Yao, Andrew C},
  booktitle={23rd Annual Symposium on Foundations of Computer Science (SFCS 1982)},
  pages={80--91},
  year={1982},
  organization={IEEE}
}


@article{marsaglia2003xorshift,
   author = {George Marsaglia},
   title = {Xorshift RNGs},
   journal = {Journal of Statistical Software, Articles},
   volume = {8},
   number = {14},
   year = {2003},
   keywords = {},
   abstract = {Description of a class of simple, extremely fast random number generators (RNGs) with periods 2k - 1 for k = 32, 64, 96, 128, 160, 192. These RNGs seem to pass tests of randomness very well.},
   issn = {1548-7660},
   pages = {1--6},
   doi = {10.18637/jss.v008.i14},
   url = {https://www.jstatsoft.org/v008/i14}
}


@article{l1999tables,
  title={Tables of linear congruential generators of different sizes and good lattice structure},
  author={L’ecuyer, Pierre},
  journal={Mathematics of Computation},
  volume={68},
  number={225},
  pages={249--260},
  year={1999}
}

@article{brown1994random,
  title={Random number generation with arbitrary strides},
  author={Brown, Forrest B},
  journal={Transactions of the American Nuclear Society},
  volume={71},
  number={CONF-941102-},
  year={1994}
}


@inproceedings {222637,
author = {Anand Padmanabha Iyer and Zaoxing Liu and Xin Jin and Shivaram Venkataraman and Vladimir Braverman and Ion Stoica},
title = {{ASAP}: Fast, Approximate Graph Pattern Mining at Scale},
booktitle = {13th {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI} 18)},
year = {2018},
isbn = {978-1-939133-08-3},
address = {Carlsbad, CA},
pages = {745--761},
url = {https://www.usenix.org/conference/osdi18/presentation/iyer},
publisher = {{USENIX} Association},
month = oct,
}

@article{pavan2013counting,
  title={Counting and sampling triangles from a graph stream},
  author={Pavan, Aduri and Tirthapura, Srikanta and others},
  year={2013}
}


@article{saito2007application,
  title={An application of finite field: Design and implementation of 128-bit instruction-based fast pseudorandom number generator},
  author={Saito, Mutsuo},
  journal={Master's thesis, Hiroshima University, Hiroshima, Japan. http://www. math. sci. hiroshima-u. ac. jp/\~{} m-mat/MT/SFMT M},
  volume={62821},
  year={2007}
}

@article{quoc2017approximate,
  title={Approximate Stream Analytics in Apache Flink and Apache Spark Streaming},
  author={Quoc, Do Le and Chen, Ruichuan and Bhatotia, Pramod and Fetze, Christof and Hilt, Volker and Strufe, Thorsten},
  journal={arXiv preprint arXiv:1709.02946},
  year={2017}
}

@inproceedings{dabal2014study,
  title={A study on fast pipelined pseudo-random number generator based on chaotic logistic map},
  author={Dabal, Pawel and Pelka, Ryszard},
  booktitle={17th International Symposium on Design and Diagnostics of Electronic Circuits \& Systems},
  pages={195--200},
  year={2014},
  organization={IEEE}
}

@inproceedings{thomas2008fpga,
  title={FPGA-optimised high-quality uniform random number generators},
  author={Thomas, David Barrie and Luk, Wayne},
  booktitle={Proceedings of the 16th international ACM/SIGDA symposium on Field programmable gate arrays},
  pages={235--244},
  year={2008}
}

@inproceedings{comer2012random,
  title={Random number generators using cellular automata implemented on FPGAs},
  author={Comer, Jonathan M and Cerda, Juan C and Martinez, Chris D and Hoe, David HK},
  booktitle={Proceedings of the 2012 44th Southeastern Symposium on System Theory (SSST)},
  pages={67--72},
  year={2012},
  organization={IEEE}
}

@inproceedings{dabal2012fpga,
  title={FPGA implementation of chaotic pseudo-random bit generators},
  author={Dabal, Pawel and Pelka, Ryszard},
  booktitle={Proceedings of the 19th International Conference Mixed Design of Integrated Circuits and Systems-MIXDES 2012},
  pages={260--264},
  year={2012},
  organization={IEEE}
}


@inproceedings{mansingka2013fibonacci,
  title={Fibonacci-based hardware post-processing for non-autonomous signum hyperchaotic system},
  author={Mansingka, Abhinav S and Barakat, Mohamed L and Zidan, M Affan and Radwan, Ahmed G and Salama, Khaled N},
  booktitle={2013 International Conference on IT Convergence and Security (ICITCS)},
  pages={1--4},
  year={2013},
  organization={IEEE}
}

@inproceedings{passerat2011pseudo,
  title={Pseudo-random number generation on GP-GPU},
  author={Passerat-Palmbach, Jonathan and Mazel, Claude and Hill, David RC},
  booktitle={2011 IEEE Workshop on Principles of Advanced and Distributed Simulation},
  pages={1--8},
  year={2011},
  organization={IEEE}
}

@article{de2018transformations,
  title={Transformations of high-level synthesis codes for high-performance computing},
  author={de Fine Licht, Johannes and Meierhans, Simon and Hoefler, Torsten},
  journal={arXiv preprint arXiv:1805.08288},
  year={2018}
}

@inproceedings{durst1989using,
  title={Using linear congruential generators for parallel random number generation},
  author={Durst, Mark J},
  booktitle={Proceedings of the 21st conference on Winter simulation},
  pages={462--466},
  year={1989}
}

@inproceedings{chi2010generating,
  title={Generating parallel random sequences via parameterizing EICGs for heterogeneous computing environments},
  author={Chi, Hongmei and Cao, Yanzhao},
  booktitle={International Conference on Computational Science and Its Applications},
  pages={409--417},
  year={2010},
  organization={Springer}
}


@manual{cuRANDguide,
  title  = "CUDA Toolkit Documentation",
  author = "Nvidia",
  url    = "https://docs.nvidia.com/cuda/curand/device-api-overview.html#performance-notes",
  year   =  "2020 (accessed November 13, 2020)"
}

@article{steele2014fast,
  title={Fast splittable pseudorandom number generators},
  author={Steele Jr, Guy L and Lea, Doug and Flood, Christine H},
  journal={ACM SIGPLAN Notices},
  volume={49},
  number={10},
  pages={453--472},
  year={2014},
  publisher={ACM New York, NY, USA}
}


==> commented/test.tex <==
%!TEX root = main.tex

\subsection{Decorrelation}\label{subsec:decorrelation}
% problem

The sequences generated by LCGs with different increments are highly linearly associated.
%
Despite there are several approaches for decorrelating two random variables, such as dynamic principal component analysis~\cite{rato2013advantage} or Cholesky matrix decomposition~\cite{kessy2018optimal,ghanem2003stochastic}, they are all based on a long sliding window to filter the generated sequences, which consumes a large amount of memory and can not be efficiently executed at run-time.

Inspired by Yao's XOR Lemma~\cite{yao1982theory}: the hardness of predication is amplified when the results of several independent instances are coupled by the exclusive disjunction~(XOR, $\oplus$).
%by combining them with independent sequences (what are the well selected sequences) with the XOR operation (hard to understand).
%
We find that it is possible to decorrelate the LCG sequences following the similar idea, a set of weak associated sequences are XORed with the LCG sequences, which are highly correlated with each other to get a serial of new independent sequences with high statistical quality.

%
An example is shown in ~\Cref{fig:decorrelation}, where $X_{a,m}^{c_1}$ and $X_{a,m}^{c_2}$  are sequences generated from the LCG through parameterization via increment (belong to $\mathbb{X}_{a,m}$).
%with same modulus and multiplier but different increments (they belong to the same LCG set $\mathbb{X}_{a,m}$).
$I$ and $J$ are the sequences generated by decorrelator (we will further discuss them in following part), and they are independent from each other ($I\indep J$).
After coupling them by XOR, the combined sequences, $Z^{1}= (X_{a,m}^{c_1} \oplus I)$ and $Z^{2}= (X_{a,m}^{c_2} \oplus J)$ are uncorrelated. The proof is provided in~\Cref{thm:1}
and~\Cref{thm:2} extended to the case of $n$ sequences.




To determine the decorrelator, we provide the theoretical constraints. We define all candidate sequences for the decorrelator belonging to a set $\mathbb{K}$, and theoretical constraints for $\mathbb{K}$ can be inferred from~\Cref{thm:2}.
\begin{align}
\forall K \in \mathbb{K} \land \forall X_{a,m} \in \mathbb{X}_{a,m} &, K \indep X_{a,m}  \label{eq:k_con_1}\\
\forall K_1 \in \mathbb{K} \land \forall K_2 \in \mathbb{K} \land K_1 &\neq K_2 , K_1 \indep K_2 \label{eq:k_con_2}
\end{align}
The first constraint is that every sequence in~$\mathbb{K}$ should be independent from the LCG generator as described in~\Cref{eq:k_con_1}. The second one is given by~\Cref{eq:k_con_2}, any pair of sequences in~$\mathbb{K}$ should also be uncorrelated from each other.
%The maximal number of independent sequences can be generated by our decorrelation approach is limited by the size of $\mathbb{X}_{a,m}$

Beyond the theoretical constraints, several practical factors should also be considered when adopting this method on FPGA platform.
Firstly, XOR operation can also reduce the statistical bias~\cite{yao1982theory}. Therefore, the sequence generated by decorrelator is not restricted to have good statistical randomness, but it should have the different type of flaws comparing with LCG algorithm.
Secondly, the decorrelator should be light weight. Specifically, multiplication should be avoid.
Finally, the decorrelator should have the approach to produce massive uncorrelated sequences, adapting to the different requirement degree of parallelism

Xorshift algorithm, which is proposed by Marsaglia in 2003, can be the best candidate for the decorrelator.
Firstly, the generation process of xorshift is completely independent from LCG, which guarantees the first theoretical constraint.
More importantly, it supports the substream method to generate long period logical sequences, which can avoid long-range correlations~\cite{haramoto2008efficient} and meets the second theoretical constraint.
Xorshift has been known to be lacking the linear complexity, while LCG has enough strength in that to guarantee the statistical quality of the finally decorrelated sequence.
Furthermore, as it is based on the binary linear recurrence, it is very simple and can be efficiently implemented on FPGA platform.
The xorshift has many variants, the details of selection and comparison of the xorshift variants will be given in~\Cref{subsec:ppu}.




\begin{theorem} \label{thm:1}

Suppose we have: $X_{a,m}^{c_1}$ and $X_{a,m}^{c_2}$ from the same LCG set $\mathbb{X}_{a,m}$, and
two independent sequences $I$, $J$, both of them are also uncorrelated with $\mathbb{X}_{a,m}$.
and the combined sequences, $Z^{1}= (X_{a,m}^{c_1} \oplus I)$, $Z^{2}= (X_{a,m}^{c_2} \oplus J)$, are independent.

\end{theorem}

\begin{proof}
    Firstly, we consider two binary uniformly distributed sequences $X$ and $Y$. Let $h(X)= 1-2X$, $h(X)$ can take the value 1 and -1 corresponding to 0 and 1 in $X$.
    Here we can turn the XOR operator to multiplication:
    \begin{align}
        h(X \oplus Y ) =h(X) \cdot h(Y)
    \end{align}
    It is easy to calculate the mathematical expectation ($E$) and the variance ($var$) of $h(X)$, also the covariance ($cov$) bewteen $h(X)$ and $h(Y)$:
    \begin{align}
        E(h(X)) &= 1 - 2E(X) \label{eq:trick_1}\\
        var(h(X)) &= 4 var(X) \label{eq:trick_2} \\
        cov(h(X),h(Y)) &= 4 cov(X, Y) \label{eq:trick_3}
    \end{align}
    As all the sequences are uniformly distributed, $E(X)$ can be close to $1/2$:
    \begin{align}
        E(X) = \mu_{X} \approx 1/2 \label{eq:e_approx}
    \end{align}
    Using $var(X) = E(X^2) - (E(X))^2$, we can approximate the variance of X following~\Cref{eq:e_approx}:
    \begin{align}
        var(X) = \mu_{X} - (\mu_{X})^2 \approx 1/4 \label{eq:approx_var}
    \end{align}
    Therefore, we can calculate the variance of the new sequence $X \oplus Y$ from~\Cref{eq:trick_2,eq:approx_var}:
    \begin{align}
        var(X \oplus Y) &= \frac{var(h(X \oplus Y))}{4} = \frac{var(h(X)) \cdot var(h(Y))}{4}   \nonumber\\
        &= 4\cdot var(X) \cdot var(Y)  \nonumber\\
        &\approx 1/4 \label{eq:approx_xor_var}
    \end{align}
    Then, from the definition, the cross-correlation of the $Z$, $\rho_{Z}$ can be represented by:
    \begin{align}
        \rho_{Z} =\frac{cov(X_{a,m}^{c_1} \oplus I, X_{a,m}^{c_2} \oplus J)}{\sqrt{var(X_{a,m}^{c_1} \oplus I) \cdot var(X_{a,m}^{c_2} \oplus J) }} \label{eq:rho}
    \end{align}
    \Cref{eq:rho} can be further approximated using~\Cref{eq:approx_xor_var}
    \begin{align}
        \rho_{Z} \approx 4 \cdot cov(X_{a,m}^{c_1} \oplus I, X_{a,m}^{c_2} \oplus J)  \label{eq:approx_var_res}
    \end{align}
    Where the covariance can be rewritten into:
    \begin{align}
         cov(&X_{a,m}^{c_1} \oplus I, X_{a,m}^{c_2} \oplus J) \nonumber\\
        &= \frac{cov[h(X_{a,m}^{c_1} \oplus I), h(X_{a,m}^{c_2} \oplus J)]}{4} \nonumber\\
        &= \frac{cov[h(X_{a,m}^{c_1}) \cdot h(I), h(X_{a,m}^{c_2}) \cdot h(J)]}{4}  \nonumber\\
        &=
        \!\begin{aligned}[t]
            &\frac{1}{4} \cdot \bigg(E[h(X_{a,m}^{c_1}) h(X_{a,m}^{c_2}) h(I) h(J)] \nonumber\\
            &- E[h(X_{a,m}^{c_1}) h(I))] E[h(X_{a,m}^{c_2}) h(J)] \bigg)
        \end{aligned}
        &\\ \label{eq:xor_simple_1}
    \end{align}
    As $X_{a,m}$ is independent of $I$ and $J$, the first item in~\Cref{eq:xor_simple_1} can be represented by their covariances:
    \begin{align}
        E[&h(X_{a,m}^{c_1}) h(X_{a,m}^{c_2}) h(I) h(J)]  \nonumber\\
        &=E[h(X_{a,m}^{c_1}) h(X_{a,m}^{c_2})] \cdot E[h(I) h(J)] \nonumber\\
        &=
        \!\begin{aligned}[t]
            &\bigg(cov[h(X_{a,m}^{c_1}),h(X_{a,m}^{c_2})] + E[h(X_{a,m}^{c_1})]E[h(X_{a,m}^{c_2})] \bigg) \nonumber\\
            &\cdot  \bigg(cov[h(I),h(J)] + E[h(I)]E[h(J)] \bigg)
        \end{aligned}
        &\\ \label{eq:cov_intermiddle}
    \end{align}
    Similar with~\Cref{eq:approx_var_res}, we use the correlation ($corr$) to replace the covariance items in~\Cref{eq:cov_intermiddle}:
    \begin{align}
        E[&h(X_{a,m}^{c_1}) h(X_{a,m}^{c_2}) h(I) h(J)]  \nonumber\\
        &\approx
        \!\begin{aligned}[t]
            &\frac{1}{4} \cdot \bigg(corr[h(X_{a,m}^{c_1}),h(X_{a,m}^{c_2})] + 4E[h(X_{a,m}^{c_1})]E[h(X_{a,m}^{c_2})] \bigg) \\
            &\cdot  \bigg(corr[h(I),h(J)] + 4E[h(I)]E[h(J)] \bigg)
        \end{aligned}
        \label{eq:corr_intermiddle}
    \end{align}
    As $X_{a,m}^{c_1}$ and $X_{a,m}^{c_2}$ from the same LCG set, the bias of their expectation can be ignored.
    \begin{align}
        E(X_{a,m}^{c_1}) = E(X_{a,m}^{c_2}) =\mu_{X_{a,m}}
    \end{align}
    Here, $\rho_{X_{a,m}}$ represents the correlation of $X_{a,m}^{c_1}$ and $X_{a,m}^{c_2}$, and $\rho_{(I,J)}$ represents the correlation of $I$ and $J$, Finally, combining ~\Cref{eq:approx_var_res,eq:xor_simple_1,eq:cov_intermiddle,eq:corr_intermiddle},~\Cref{eq:rho} can be simplified as:
    \begin{align}
       \rho_{Z} &\approx \rho_{X_{a,m}} \cdot \rho_{(I,J)} + \rho_{X_{a,m}} \cdot (1 - 2\mu_{(I,J)}) \nonumber\\
                &+ \rho_{(I,J)} \cdot (1 - 2\mu_{X_{a,m}})
        \label{eq:final}
    \end{align}
    From the conditions: $I$ is independent from $J$, it obvious that $\rho_{(I,J)}$ is close to zero. Therefore, the first item in~\Cref{eq:final} can be treated as zero even $\rho_{X_{a,m}}$ is close to 1 ($X_{a,m}^{c_1}$ and $X_{a,m}^{c_2}$ are highly correlated). From~\Cref{eq:e_approx}, $\mu_{X_{a,m}}$ and $\mu_{(I,J)}$ is close to $1/2$, the second and third item can be neglected. Hence,
    $\rho_{Z}$ is proven to be close to zero, and it indicates that the two coupled sequences are uncorrelated from each other.

\end{proof}





\begin{theorem} \label{thm:2}

Supposing there is a set of independent sequences $\mathbb{K}$, of which all members are uncorrelated with $\mathbb{X}_{a,m}$.
Separately selecting $n$ sequences~$(n>2)$, $\{K^i\}_{i=1}^{n}$ from $\mathbb{K}$, and $\{X_{a,m}^{c_i}\}_{i=1}^{n}$ from $\mathbb{X}_{a,m}$, then, the combined sequences, $\{Z^{i}= X_{a,m}^{c_i} \oplus K^i\}_{i=1}^{n}$ are pairwise independent from each other.

\end{theorem}

\begin{proof}

Let $P(n)$ be the statement "the $n$ decorrelated sequences, $\{Z^{i}= X_{a,m}^{c_i} \oplus K^i\}_{i=1}^{n}$ are pairwise independent", We will prove by induction that $P(n)$ holds for all $n>2$,from which the theorem follows.

For the base case, we prove $P(3)$, three distinct sequences are pairwise independent (assuming they are $Z^1$, $Z^2$ and $Z^3$).
%
From the definition, We have and $Z^2 =X_{a,m}^{c_2} \oplus K^2$, As $K^1$ and $K^2$ belong to $\mathbb{K}$, which is a set of pairwise independent sequences.

For the inductive step, assuming that $P(j)$ is true, we will prove that $P(j + 1)$ is also true. Comparing with $P(j)$, $Z^{j + 1}$ is the new introduced sequence, of which the $K^{j+1}$ is independent with the sequences in $\{K^i\}_{i=1}^{j}$. Adopting~\Cref{thm:1}, the new sequence  $Z^{j + 1}$ can be independent with all the member in $\{Z^{i}\}_{i=1}^{j}$, which are pairwise independent in $P(j)$. Therefore, by the definition of pairwise independence,  $P(j+1)$ is true, completing the induction.

\end{proof}


% To maximize the period, the selection of $a$ and $c$ should follow the Hull-Dobell Theorems~\cite{hull1962random}.
%The period of LCG, $p$, . The period is an important property of a generation algorithm, and it should be much longer than any sequence that will be used in any application.
%If $c = 0$, the generator is called as a multiplicative congruential generator (MCG).
%When $c\neq0$, the new sequence can be affinely transformed from the MCG~\cite{steele2020computationally}.
%The selection of to maximize the period, which is defined as
%The formula shows that the calculation of one output of LCG only need one multiplication and one addition, which can be efficiently mapped to multiply–accumulate (MAC) hardware unit.
%Hence, if the state width is not very large, LCG can be efficiently implemented on modern processors which supports MAC instructions.


==> packagelist.tex <==
%\usepackage{framed,multirow}
\usepackage{amssymb}
\usepackage{latexsym}
% Following three lines are needed for this document.
% If you are not loading colors or url, then these are
% not required.
\usepackage{url}
\usepackage{xcolor}
\definecolor{newcolor}{rgb}{.8,.349,.1}

\usepackage{soul}
% \usepackage{caption}

%ours packages
% font
%\usepackage{times}
\usepackage{epsfig}
\usepackage{amssymb}
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}
% math
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{cases}
\usepackage{esint}
% figures
\usepackage{graphicx}
\usepackage{subfig}
% algorithm
\usepackage{algorithm} %format of the algorithm
\usepackage{algorithmic} %format of the algorithm
\usepackage{multirow} %multirow for format of Table
\usepackage{amsmath}
\usepackage{xcolor}

%\usepackage{natbib}
%\usepackage[square,sort,comma,numbers]{natbib}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newtheorem{thm}{Theorem}
% table
%\usepackage{tabularx}
%\usepackage{natbib}
\usepackage{makecell}
\usepackage[normalem]{ulem}
\usepackage{overpic}

% revision
\newcommand{\rev}[1]{\textcolor{blue}{#1}}
% \newcommand{\rev}[1]{#1}

% commends
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\sectionref}[1]{Section~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~(\ref{#1})}
% \newcommand{\eqref}[1]{Eq.~(\ref{#1})}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\sArt}[0]{state-of-the-art}
% \newcommand{\gc}[1]{\textcolor{blue}{\{#1\}}}
\newcommand{\gc}[1]{}
\newcommand{\gcc}[1]{\textcolor{red}{#1}}
% \newcommand{\gcc}[1]{#1}
\newcommand{\lenetimp}[0]{$\textbf{0.52\%}$}
\newcommand{\vggimp}[0]{$\textbf{3.10\%}$}
\newcommand{\alexnetOimp}[0]{$\textbf{2.29\%}$}
\newcommand{\alexnetFimp}[0]{$\textbf{0.35\%}$}
\newcommand{\resnetOimp}[0]{$\textbf{2.47\%}$}
\newcommand{\resnetFimp}[0]{$\textbf{1.40\%}$}
\newcommand{\mobileOimp}[0]{$\textbf{2.57\%}$}
\newcommand{\mobileFimp}[0]{$\textbf{1.64\%}$}

% table
\usepackage{array}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}

==> tools/mycrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__

